Inflation with sterile scalar coupled to massive fermions and to gravity

In the recent paper [3] it was shown that the consistency of the quantum theory of a sterile scalar coupled to massive fermions requires the inclusion of odd-power terms in the potential of scalar self-interaction. One of the most important examples of a sterile scalar is the inflaton, that is typically a real scalar field which does not belong to representations of particle physics gauge groups, such as $SU(2)$. Here we explore the effects of the odd-power terms in the inflaton potential on main observables, such as the scalar spectral index $n_s$ and the tensor-to-scalar ratio $r$, in the case of a strong, non-minimal coupling of the inflaton to gravity.

==> preamble.tex <==
%% preamble.tex

%\documentclass[11pt,fleqn]{article}
\usepackage{amsfonts,amssymb,cite}
\usepackage{graphicx}

%\input preamble.tex
%\begin{document}
%\twocolumn[
%\jnumber{}{}

		%% PAGE SETUP AND TITLE BLOCK %%

\topmargin -10mm
\oddsidemargin -6mm
\evensidemargin -12mm
\textheight 242mm
\textwidth 178mm
\emergencystretch 6pt
\mathsurround 1pt
\mathindent 1em
\columnsep 8mm
\pagestyle{myheadings}
\newcommand{\bls}[1]{\renewcommand{\baselinestretch}{#1}}
\def\onecol{\onecolumn \mathindent 2em}
\def\twocol{\twocolumn \mathindent 1em}
\def\noi{\noindent}
\def\jnumber#1#2{\thispagestyle{empty} \noi\unitlength=1mm
    	\begin{picture}(178,10)
            \put(177,15){\llap{\large\it Grav. Cosmol. No.\,#1, #2}}
                    \end{picture}}

\newcommand{\Title}[1]{\noi {{\Large\bf #1}}\\[1ex]}

\newcommand{\Author}[2]{\noi{\bf #1}\\[2ex]\noi{\normalsize\it #2}\\}

\def\Aunames#1{\noi{\bf #1}}
\def\au#1{${}^{#1}$}
\def\Addresses#1{\medskip\noi \protect
	\begin{description}\itemsep -3pt {\it #1} \end{description}}
\def\adr#1#2{\item[${}^{#1}$]{\it #2}}

\newcommand{\Rec}[1]{\noi {\it Received #1} \\}
\newcommand{\Recfin}[1]{\noi {\it Received in final form #1} \\}
\newcommand{\Dates}[3]{\noi {\it Received #1}\\
		          \noi {\it Received in final form #2}\\			
		          \noi {\it Accepted #3}\\} 
\newcommand{\Abstract}[1]{\vskip 2mm \begin{center}
        \parbox{16.4cm}{\small\noi #1} \end{center}\medskip}
\newcommand{\foom}[1]{\protect\footnotemark[#1]}
\newcommand{\foox}[2]{\footnotetext[#1]{#2}\addtocounter{footnote}{1}}
\def\email#1#2{\footnotetext[#1]{e-mail: #2}\addtocounter{footnote}{1}}

		%%  TEXT AND SPACES %%

\def\nq{\hspace*{-1em}}
\def\nqq{\hspace*{-2em}}
\def\nhq{\hspace*{-0.5em}}
\def\nhh{\hspace*{-0.3em}}
\def\qq{\qquad}
\def\cm{\hspace*{1cm}}
\def\inch{\hspace*{1in}}
\def\wide{\mbox{$\dst\vphantom{\int}$}}
\def\Wide{\mbox{$\dst\vphantom{\intl_a^a}$}}
\def\ten#1{\mbox{$\times 10^{#1}$}}
\def\deg{\mbox{${}^\circ$}}                     %% degree
\def\degC{\mbox{${}^\circ$C}}                %% Celsius degree
\def\uml#1{\"{#1}}                                   % Umlaut
% ---------------------
\usepackage{color}
\def\red#1{{\color{red} #1}}
\def\blue#1{{\color{blue} #1}}
% ---------------------

		%% FIGURES %%

\def\floatpagefraction{.95}
\def\topfraction{.95}
\def\bottomfraction{.95}
\def\textfraction{.05}
\def\dblfloatpagefraction{.95}
\def\dbltopfraction{.95}

\newcommand{\NFigure}[3]{\begin{figure} \centering   % Narrow figure
        \includegraphics[scale=#2]{#1}                        % #1 = figure file
        \caption{\protect\small #3}                              % #2 = size fraction     
	\end{figure}}                                            % #3 = caption

\newcommand{\WFigure}[3]{\begin{figure*} \centering  % Wide figure
        \includegraphics[scale=#2]{#1}
        \caption{\protect\small #3}
	\end{figure*}}

		%% END GROUP %%

\def\Acknow#1{\subsection*{Acknowledgments} #1}
\def\Funding#1{\subsection*{Funding} #1}
\def\ConflictHe{\subsection*{Conflict of interest} 
	The author declares that he has no conflicts of interest.}
\def\ConflictShe{\subsection*{Conflict of interest} 
	The author declares that she has no conflicts of interest.}
\def\ConflictThey{\subsection*{Conflict of interest} 
	The authors declare that they have no conflicts of interest.}

%% References
\def\Jl#1#2{#1 {\bf #2},\ }

\def\ApJ#1 {\Jl{Astroph. J.}{#1}}
\def\CQG#1 {\Jl{Class. Quantum Grav.}{#1}}
\def\DAN#1 {\Jl{Dokl. AN SSSR}{#1}}
\def\GC#1 {\Jl{Grav. Cosmol.}{#1}}
\def\GRG#1 {\Jl{Gen. Rel. Grav.}{#1}}
\def\IJMPD#1 {\Jl{Int. J. Mod. Phys. D}{#1}}
\def\JETF#1 {\Jl{Zh. Eksp. Teor. Fiz.}{#1}}
\def\JETP#1 {\Jl{Sov. Phys. JETP}{#1}}
\def\JHEP#1 {\Jl{JHEP}{#1}}
\def\JMP#1 {\Jl{J. Math. Phys.}{#1}}
\def\NPB#1 {\Jl{Nucl. Phys. B}{#1}}
\def\NP#1 {\Jl{Nucl. Phys.}{#1}}
\def\PLA#1 {\Jl{Phys. Lett. A}{#1}}
\def\PLB#1 {\Jl{Phys. Lett. B}{#1}}
\def\PRD#1 {\Jl{Phys. Rev. D}{#1}}
\def\PRL#1 {\Jl{Phys. Rev. Lett.}{#1}}

		%% EQUATIONS %%

%% aligning, numbering
\def\al{&\nhq}
\def\lal{&&\nqq {}}
\def\eq{Eq.\,}
\def\eqs{Eqs.\,}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\bear{\begin{eqnarray}}
\def\bearr{\begin{eqnarray} \lal}
\def\ear{\end{eqnarray}}
\def\earn{\nonumber \end{eqnarray}}
\def\nn{\nonumber\\ {}}
\def\nnv{\nonumber\\[5pt] {}}
\def\nnn{\nonumber\\ \lal }
\def\nnnv{\nonumber\\[5pt] \lal }
\def\yy{\\[5pt] {}}
\def\yyy{\\[5pt] \lal }
\def\eql{\al =\al}
\def\eqv{\al \equiv \al}
\def\sequ#1{\setcounter{equation}{#1}}

%% fractions

\def\dst{\displaystyle}
\def\tst{\textstyle}
\def\fracd#1#2{{\dst\frac{#1}{#2}}}
\def\fract#1#2{{\tst\frac{#1}{#2}}}
\def\Half{{\fracd{1}{2}}}
\def\half{{\fract{1}{2}}}

%% other

\def\e{{\,\rm e}}
\def\d{\partial}
\def\re{\mathop{\rm Re}\nolimits}
\def\im{\mathop{\rm Im}\nolimits}
\def\arg{\mathop{\rm arg}\nolimits}
\def\tr{\mathop{\rm tr}\nolimits}
\def\sign{\mathop{\rm sign}\nolimits}
\def\diag{\mathop{\rm diag}\nolimits}
\def\dim{\mathop{\rm dim}\nolimits}
\def\const{{\rm const}}
\def\eps{\varepsilon}
\def\ep{\epsilon}

\def\then{\ \Rightarrow\ }
\newcommand{\toas}{\mathop {\ \longrightarrow\ }\limits }
\newcommand{\aver}[1]{\langle \, #1 \, \rangle \mathstrut}
\newcommand{\vars}[1]{\left\{\begin{array}{ll}#1\end{array}\right.}
\def\suml{\sum\limits}
\def\intl{\int\limits}

%% Author's definitions

%\addtolength{\textheight}{1cm}
%\bls{1.0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{document}
%\thispagestyle{empty}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








